Question Answering over Knowledge Base using Language Model Embeddings

Knowledge Base, represents facts about the world, often in some form of subsumption ontology, rather than implicitly, embedded in procedural code, the way a conventional computer program does. While there is a rapid growth in knowledge bases, it poses a challenge of retrieving information from them. Knowledge Base Question Answering is one of the promising approaches for extracting substantial knowledge from Knowledge Bases. Unlike web search, Question Answering over a knowledge base gives accurate and concise results, provided that natural language questions can be understood and mapped precisely to an answer in the knowledge base. However, some of the existing embedding-based methods for knowledge base question answering systems ignore the subtle correlation between the question and the Knowledge Base (e.g., entity types, relation paths, and context) and suffer from the Out Of Vocabulary problem. In this paper, we focused on using a pre-trained language model for the Knowledge Base Question Answering task. Firstly, we used Bert base uncased for the initial experiments. We further fine-tuned these embeddings with a two-way attention mechanism from the knowledge base to the asked question and from the asked question to the knowledge base answer aspects. Our method is based on a simple Convolutional Neural Network architecture with a Multi-Head Attention mechanism to represent the asked question dynamically in multiple aspects. Our experimental results show the effectiveness and the superiority of the Bert pre-trained language model embeddings for question answering systems on knowledge bases over other well-known embedding methods.

==> refer.tex <==
@article{DBLP:journals/corr/VaswaniSPUJGKP17,
  author    = {Ashish Vaswani and
               Noam Shazeer and
               Niki Parmar and
               Jakob Uszkoreit and
               Llion Jones and
               Aidan N. Gomez and
               Lukasz Kaiser and
               Illia Polosukhin},
  title     = {Attention Is All You Need},
  journal   = {CoRR},
  volume    = {abs/1706.03762},
  year      = {2017},
  url       = {http://arxiv.org/abs/1706.03762},
  archivePrefix = {arXiv},
  eprint    = {1706.03762},
  timestamp = {Mon, 13 Aug 2018 16:48:37 +0200},
  biburl    = {https://dblp.org/rec/bib/journals/corr/VaswaniSPUJGKP17},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}
@inproceedings{inproceedings,
author = {Chardin, Brice and Coquery, Emmanuel and PAILLOUX, Marie and Petit, Jean-Marc},
year = {2014},
month = {12},
pages = {1203-1206},
title = {RQL: A SQL-like query language for discovering meaningful rules},
volume = {2014},
journal = {IEEE International Conference on Data Mining (demonstration)},
doi = {10.1109/ICDMW.2014.50}
}
@article{rajpurkar2016squad,
  title={Squad: 100,000+ questions for machine comprehension of text},
  author={Rajpurkar, Pranav and Zhang, Jian and Lopyrev, Konstantin and Liang, Percy},
  journal={arXiv preprint arXiv:1606.05250},
  year={2016}
}
@article{Wolf2019HuggingFacesTS,
  title={HuggingFace's Transformers: State-of-the-art Natural Language Processing},
  author={Thomas Wolf and Lysandre Debut and Victor Sanh and Julien Chaumond and Clement Delangue and Anthony Moi and Pierric Cistac and Tim Rault and R'emi Louf and Morgan Funtowicz and Jamie Brew},
  journal={ArXiv},
  year={2019},
  volume={abs/1910.03771}
}

@article{klyne2009resource,
  title={Resource description framework (rdf): concepts and abstract syntax, 2004},
  author={Klyne, Graham and Carroll, Jeremy J and McBride, B},
  journal={February. URL: http://www. w3. org/TR/2004/REC-rdf-concepts-20040210},
  year={2009}
}

@article{kingma2014adam,
  title={Adam: A method for stochastic optimization},
  author={Kingma, Diederik P and Ba, Jimmy},
  journal={arXiv preprint arXiv:1412.6980},
  year={2014}
}

@article{devlin2018bert,
  title={Bert: Pre-training of deep bidirectional transformers for language understanding},
  author={Devlin, Jacob and Chang, Ming-Wei and Lee, Kenton and Toutanova, Kristina},
  journal={arXiv preprint arXiv:1810.04805},
  year={2018}
}

@article{kim2014convolutional,
  title={Convolutional neural networks for sentence classification},
  author={Kim, Yoon},
  journal={arXiv preprint arXiv:1408.5882},
  year={2014}
}

@article{singhal2012introducing,
  title={Introducing the knowledge graph: things, not strings},
  author={Singhal, Amit},
  journal={Official google blog},
  volume={16},
  year={2012}
}

 @inproceedings{10.1145/1242572.1242667,
 author = {Suchanek, Fabian M. and Kasneci, Gjergji and Weikum, Gerhard},
 title = {Yago: A Core of Semantic Knowledge},
 year = {2007},
 isbn = {9781595936547},
 publisher = {Association for Computing Machinery},
 address = {New York, NY, USA},
 url = {https://doi.org/10.1145/1242572.1242667},
 doi = {10.1145/1242572.1242667},
 booktitle = {Proceedings of the 16th International Conference on World Wide Web},
 pages = {697–706},
 numpages = {10},
 keywords = {WordNet, wikipedia},
 location = {Banff, Alberta, Canada},
 series = {WWW ’07}
}
@article{winograd1983language,
  title={Language as a cognitive process: Volume 1: Syntax},
  author={Winograd, Terry},
  year={1983},
  publisher={Addison-Wesley Pub. Co., Reading, MA}
}

@article{peters2018deep,
  title={Deep contextualized word representations},
  author={Peters, Matthew E and Neumann, Mark and Iyyer, Mohit and Gardner, Matt and Clark, Christopher and Lee, Kenton and Zettlemoyer, Luke},
  journal={arXiv preprint arXiv:1802.05365},
  year={2018}
}

@article{radford2019language,
  title={Language models are unsupervised multitask learners},
  author={Radford, Alec and Wu, Jeffrey and Child, Rewon and Luan, David and Amodei, Dario and Sutskever, Ilya},
  journal={OpenAI Blog},
  volume={1},
  number={8},
  pages={9},
  year={2019}
}
@InProceedings{10.1007/978-3-642-77189-7_5,
author="Sag, Ivan A.",
editor="Klein, Ewan
and Veltman, Frank",
title="Linguistic Theory and Natural Language Processing",
booktitle="Natural Language and Speech",
year="1991",
publisher="Springer Berlin Heidelberg",
address="Berlin, Heidelberg",
pages="69--83",
abstract="The 1960's were a tempestuous time --- a time of rebellion, a time for defining new directions. And by the end of the 1960's the field of `theoretical' Linguistics had already rebelled and defined its new direction --- a path directly away from the field of Natural Language Processing (NLP) and away from Psycholinguistics. Following Chomsky's lead, linguists showed little interest in `engineering applications' like NLP.2 And once psycholinguistic studies began to contradict the transformational theories of the time (e.g. by finding that transformational complexity was often at odds with measurable real-time processing complexity), it was the psycholinguistic methods, not the linguistic theories that were dismissed. Down to the present day, most people who call themselves `theoretical' linguists are in complete agreement that processing considerations have little or no role to play in the development of theories of linguistic knowledge. The `best theory', it is believed, will emerge from considerations of elegance alone: the succinct expression of `linguistically significant generalizations'.",
isbn="978-3-642-77189-7"
}

@InProceedings{10.1007/978-3-540-27775-0_33,
author="Bry, Fran{\c{c}}ois
and P{\u{a}}tr{\^a}njan, Paula-Lavinia
and Schaffert, Sebastian",
editor="Demoen, Bart
and Lifschitz, Vladimir",
title="Xcerpt and XChange -- Logic Programming Languages for Querying and Evolution on the Web",
booktitle="Logic Programming",
year="2004",
publisher="Springer Berlin Heidelberg",
address="Berlin, Heidelberg",
pages="450--451",
abstract="The Semantic Web is an endeavor aiming at enriching the existing Web with meta-data and data (and meta-data) processing so as to allow computer systems to actually reason with the data instead of merely rendering it. To this aim, it is necessary to be able to query and update data and meta-data. Existing Semantic Web query languages (like DQL) are special purpose, they are not capable of processing generic Web data. On the other hand, the language Xcerpt [1,2] presented in the poster is a general purpose language that can query any kind of XML data and at the same time, being based on logic programming, provides advanced reasoning capabilities. Likewise, the maintenance and evolution of data on the (Semantic) Web is necessary: the Web is a ''living organism'' whose dynamic character requires languages for specifying its evolution. This requirement regards not only updating data from Web resources, but also the propagation of changes on the Web. These issues have not received much attention so far, existing update languages (e.g. XML-RL Update Language [3]) and reactive languages [4] for the Web offer the possibility to execute simple update operations and, moreover, important features needed for propagation of updates on the Web are still missing. The language XChange also presented in the poster builds upon the query language Xcerpt and provides advanced, Web-specific capabilities, such as propagation of changes on the Web (change) and event-based communications between Web sites (exchange).",
isbn="978-3-540-27775-0"
}



@article{harris1954distributional,
  title={Distributional structure},
  author={Harris, Zellig S},
  journal={Word},
  volume={10},
  number={2-3},
  pages={146--162},
  year={1954},
  publisher={Taylor \& Francis}
}

@inproceedings{hao-etal-2017-end,
    title = "An End-to-End Model for Question Answering over Knowledge Base with Cross-Attention Combining Global Knowledge",
    author = "Hao, Yanchao  and
      Zhang, Yuanzhe  and
      Liu, Kang  and
      He, Shizhu  and
      Liu, Zhanyi  and
      Wu, Hua  and
      Zhao, Jun",
    booktitle = "Proceedings of the 55th Annual Meeting of the Association for Computational Linguistics (Volume 1: Long Papers)",
    month = jul,
    year = "2017",
    address = "Vancouver, Canada",
    publisher = "Association for Computational Linguistics",
    url = "https://www.aclweb.org/anthology/P17-1021",
    doi = "10.18653/v1/P17-1021",
    pages = "221--231",
    abstract = "With the rapid growth of knowledge bases (KBs) on the web, how to take full advantage of them becomes increasingly important. Question answering over knowledge base (KB-QA) is one of the promising approaches to access the substantial knowledge. Meanwhile, as the neural network-based (NN-based) methods develop, NN-based KB-QA has already achieved impressive results. However, previous work did not put more emphasis on question representation, and the question is converted into a fixed vector regardless of its candidate answers. This simple representation strategy is not easy to express the proper information in the question. Hence, we present an end-to-end neural network model to represent the questions and their corresponding scores dynamically according to the various candidate answer aspects via cross-attention mechanism. In addition, we leverage the global knowledge inside the underlying KB, aiming at integrating the rich KB information into the representation of the answers. As a result, it could alleviates the out-of-vocabulary (OOV) problem, which helps the cross-attention model to represent the question more precisely. The experimental results on WebQuestions demonstrate the effectiveness of the proposed approach.",
}

@inproceedings{bollacker2008freebase,
  title={Freebase: a collaboratively created graph database for structuring human knowledge},
  author={Bollacker, Kurt and Evans, Colin and Paritosh, Praveen and Sturge, Tim and Taylor, Jamie},
  booktitle={Proceedings of the 2008 ACM SIGMOD international conference on Management of data},
  pages={1247--1250},
  year={2008},
  organization={AcM}
}

@article{bahdanau2014neural,
  title={Neural machine translation by jointly learning to align and translate},
  author={Bahdanau, Dzmitry and Cho, Kyunghyun and Bengio, Yoshua},
  journal={arXiv preprint arXiv:1409.0473},
  year={2014}
}

@article{rush2015neural,
  title={A neural attention model for abstractive sentence summarization},
  author={Rush, Alexander M and Chopra, Sumit and Weston, Jason},
  journal={arXiv preprint arXiv:1509.00685},
  year={2015}
}

@article{yin2016simple,
  title={Simple question answering by attentive convolutional neural network},
  author={Yin, Wenpeng and Yu, Mo and Xiang, Bing and Zhou, Bowen and Sch{\"u}tze, Hinrich},
  journal={arXiv preprint arXiv:1606.03391},
  year={2016}
}

@inproceedings{hochreiter1997lstm,
  title={LSTM can solve hard long time lag problems},
  author={Hochreiter, Sepp and Schmidhuber, J{\"u}rgen},
  booktitle={Advances in neural information processing systems},
  pages={473--479},
  year={1997}
}

@article{sutskever2014sequence,
  title={Sequence to sequence learning with neural networks},
  author={Sutskever, I and Vinyals, O and Le, QV},
  journal={Advances in NIPS},
  year={2014}
}

@article{dyer2015transition,
  title={Transition-based dependency parsing with stack long short-term memory},
  author={Dyer, Chris and Ballesteros, Miguel and Ling, Wang and Matthews, Austin and Smith, Noah A},
  journal={arXiv preprint arXiv:1505.08075},
  year={2015}
}
@inproceedings{berant-etal-2013-semantic,
    title = "Semantic Parsing on {F}reebase from Question-Answer Pairs",
    author = "Berant, Jonathan  and
      Chou, Andrew  and
      Frostig, Roy  and
      Liang, Percy",
    booktitle = "Proceedings of the 2013 Conference on Empirical Methods in Natural Language Processing",
    month = oct,
    year = "2013",
    address = "Seattle, Washington, USA",
    publisher = "Association for Computational Linguistics",
    url = "https://www.aclweb.org/anthology/D13-1160",
    pages = "1533--1544",
}



@article{cui2017kbqa,
  title={KBQA: learning question answering over QA corpora and knowledge bases},
  author={Cui, Wanyun and Xiao, Yanghua and Wang, Haixun and Song, Yangqiu and Hwang, Seung-won and Wang, Wei},
  journal={Proceedings of the VLDB Endowment},
  volume={10},
  number={5},
  pages={565--576},
  year={2017},
  publisher={VLDB Endowment}
}

@article{hochreiter1997long,
  title={Long short-term memory},
  author={Hochreiter, Sepp and Schmidhuber, J{\"u}rgen},
  journal={Neural computation},
  volume={9},
  number={8},
  pages={1735--1780},
  year={1997},
  publisher={MIT Press}
}

@inproceedings{zhu2015aligning,
  title={Aligning books and movies: Towards story-like visual explanations by watching movies and reading books},
  author={Zhu, Yukun and Kiros, Ryan and Zemel, Rich and Salakhutdinov, Ruslan and Urtasun, Raquel and Torralba, Antonio and Fidler, Sanja},
  booktitle={Proceedings of the IEEE international conference on computer vision},
  pages={19--27},
  year={2015}
}

@inproceedings{alshawi1989logical,
  title={Logical forms in the core language engine},
  author={Alshawi, Hiyan and van Eijck, Jan},
  booktitle={27th Annual Meeting of the Association for Computational Linguistics},
  pages={25--32},
  year={1989}
}
@inproceedings{bordes2014open,
  title={Open question answering with weakly supervised embedding models},
  author={Bordes, Antoine and Weston, Jason and Usunier, Nicolas},
  booktitle={Joint European conference on machine learning and knowledge discovery in databases},
  pages={165--180},
  year={2014},
  organization={Springer}
}

@inproceedings{hao2017end,
  title={An end-to-end model for question answering over knowledge base with cross-attention combining global knowledge},
  author={Hao, Yanchao and Zhang, Yuanzhe and Liu, Kang and He, Shizhu and Liu, Zhanyi and Wu, Hua and Zhao, Jun},
  booktitle={Proceedings of the 55th Annual Meeting of the Association for Computational Linguistics (Volume 1: Long Papers)},
  pages={221--231},
  year={2017}
}
@article{hu2017answering,
  title={Answering natural language questions by subgraph matching over knowledge graphs},
  author={Hu, Sen and Zou, Lei and Yu, Jeffrey Xu and Wang, Haixun and Zhao, Dongyan},
  journal={IEEE Transactions on Knowledge and Data Engineering},
  volume={30},
  number={5},
  pages={824--837},
  year={2017},
  publisher={IEEE}
}

@article{yu2018qanet,
  title={Qanet: Combining local convolution with global self-attention for reading comprehension},
  author={Yu, Adams Wei and Dohan, David and Luong, Minh-Thang and Zhao, Rui and Chen, Kai and Norouzi, Mohammad and Le, Quoc V},
  journal={arXiv preprint arXiv:1804.09541},
  year={2018}
}

@article{weston2014memory,
  title={Memory networks},
  author={Weston, Jason and Chopra, Sumit and Bordes, Antoine},
  journal={arXiv preprint arXiv:1410.3916},
  year={2014}
}

@inproceedings{jain2016question,
  title={Question answering over knowledge base using factual memory networks},
  author={Jain, Sarthak},
  booktitle={Proceedings of the NAACL Student Research Workshop},
  pages={109--115},
  year={2016}
}

@article{bordes2014question,
  title={Question answering with subgraph embeddings},
  author={Bordes, Antoine and Chopra, Sumit and Weston, Jason},
  journal={arXiv preprint arXiv:1406.3676},
  year={2014}
}

@article{bordes2015large,
  title={Large-scale simple question answering with memory networks},
  author={Bordes, Antoine and Usunier, Nicolas and Chopra, Sumit and Weston, Jason},
  journal={arXiv preprint arXiv:1506.02075},
  year={2015}
}

@inproceedings{petroni2019language,
  title={Language Models as Knowledge Bases?},
  author={F. Petroni, T. Rockt{\"{a}}schel, A. H. Miller, P. Lewis, A. Bakhtin, Y. Wu and S. Riedel},
  booktitle={To Appear in: Proceedings of the 2019 Conference on Empirical Methods in Natural Language Processing (EMNLP), 2019},
  year={2019}
}


@inproceedings{unger2014introduction,
  title={An introduction to question answering over linked data},
  author={Unger, Christina and Freitas, Andr{\'e} and Cimiano, Philipp},
  booktitle={Reasoning Web International Summer School},
  pages={100--140},
  year={2014},
  organization={Springer}
}
@inproceedings{yih2014semantic,
  title={Semantic parsing for single-relation question answering},
  author={Yih, Wen-tau and He, Xiaodong and Meek, Christopher},
  booktitle={Proceedings of the 52nd Annual Meeting of the Association for Computational Linguistics (Volume 2: Short Papers)},
  pages={643--648},
  year={2014}
}
@article{yih2015semantic,
  title={Semantic parsing via staged query graph generation: Question answering with knowledge base},
  author={Yih, Scott Wen-tau and Chang, Ming-Wei and He, Xiaodong and Gao, Jianfeng},
  year={2015}
}

@inproceedings{zettlemoyer2009learning,
  title={Learning context-dependent mappings from sentences to logical form},
  author={Zettlemoyer, Luke S and Collins, Michael},
  booktitle={Proceedings of the Joint Conference of the 47th Annual Meeting of the ACL and the 4th International Joint Conference on Natural Language Processing of the AFNLP: Volume 2-Volume 2},
  pages={976--984},
  year={2009},
  organization={Association for Computational Linguistics}
}

@article{zettlemoyer2012learning,
  title={Learning to map sentences to logical form: Structured classification with probabilistic categorial grammars},
  author={Zettlemoyer, Luke S and Collins, Michael},
  journal={arXiv preprint arXiv:1207.1420},
  year={2012}
}

@inproceedings{yao2014information,
  title={Information extraction over structured data: Question answering with freebase},
  author={Yao, Xuchen and Van Durme, Benjamin},
  booktitle={Proceedings of the 52nd Annual Meeting of the Association for Computational Linguistics (Volume 1: Long Papers)},
  pages={956--966},
  year={2014}
}

@inproceedings{xu-etal-2016-hybrid,
    title = "Hybrid Question Answering over Knowledge Base and Free Text",
    author = "Xu, Kun  and
      Feng, Yansong  and
      Huang, Songfang  and
      Zhao, Dongyan",
    booktitle = "Proceedings of {COLING} 2016, the 26th International Conference on Computational Linguistics: Technical Papers",
    month = dec,
    year = "2016",
    address = "Osaka, Japan",
    publisher = "The COLING 2016 Organizing Committee",
    url = "https://www.aclweb.org/anthology/C16-1226",
    pages = "2397--2407",
    abstract = "Recent trend in question answering (QA) systems focuses on using structured knowledge bases (KBs) to find answers. While these systems are able to provide more precise answers than information retrieval (IR) based QA systems, the natural incompleteness of KB inevitably limits the question scope that the system can answer. In this paper, we present a hybrid question answering (hybrid-QA) system which exploits both structured knowledge base and free text to answer a question. The main challenge is to recognize the meaning of a question using these two resources, i.e., structured KB and free text. To address this, we map relational phrases to KB predicates and textual relations simultaneously, and further develop an integer linear program (ILP) model to infer on these candidates and provide a globally optimal solution. Experiments on benchmark datasets show that our system can benefit from both structured KB and free text, outperforming the state-of-the-art systems.",
}

@article{sak2014long,
  title={Long short-term memory recurrent neural network architectures for large scale acoustic modeling},
  author={Sak, Hasim and Senior, Andrew W and Beaufays, Fran{\c{c}}oise},
  year={2014}
}

@article{wang2016machine,
  title={Machine comprehension using match-lstm and answer pointer},
  author={Wang, Shuohang and Jiang, Jing},
  journal={arXiv preprint arXiv:1608.07905},
  year={2016}
}

@article{seo2016bidirectional,
  title={Bidirectional attention flow for machine comprehension},
  author={Seo, Minjoon and Kembhavi, Aniruddha and Farhadi, Ali and Hajishirzi, Hannaneh},
  journal={arXiv preprint arXiv:1611.01603},
  year={2016}
}

@article{xiong2016dynamic,
  title={Dynamic coattention networks for question answering},
  author={Xiong, Caiming and Zhong, Victor and Socher, Richard},
  journal={arXiv preprint arXiv:1611.01604},
  year={2016}
}

@article{cleeremans1989finite,
  title={Finite state automata and simple recurrent networks},
  author={Cleeremans, Axel and Servan-Schreiber, David and McClelland, James L},
  journal={Neural computation},
  volume={1},
  number={3},
  pages={372--381},
  year={1989},
  publisher={MIT Press}
}

@article{chen2019bidirectional,
  title={Bidirectional attentive memory networks for question answering over knowledge bases},
  author={Chen, Yu and Wu, Lingfei and Zaki, Mohammed J},
  journal={arXiv preprint arXiv:1903.02188},
  year={2019}
}

@article{fukushima1988neocognitron,
  title={Neocognitron: A hierarchical neural network capable of visual pattern recognition},
  author={Fukushima, Kunihiko},
  journal={Neural networks},
  volume={1},
  number={2},
  pages={119--130},
  year={1988},
  publisher={Elsevier}
}

 @inproceedings{10.5555/1986079.1986220,
 author = {Graves, Alex and Fern\'{a}ndez, Santiago and Schmidhuber, J\"{u}rgen},
 title = {Bidirectional LSTM Networks for Improved Phoneme Classification and Recognition},
 year = {2005},
 isbn = {3540287558},
 publisher = {Springer-Verlag},
 address = {Berlin, Heidelberg},
 booktitle = {Proceedings of the 15th International Conference on Artificial Neural Networks: Formal Models and Their Applications - Volume Part II},
 pages = {799–804},
 numpages = {6},
 location = {Warsaw, Poland},
 series = {ICANN’05}
}

@inproceedings{dong-etal-2015-question,
    title = "Question Answering over {F}reebase with Multi-Column Convolutional Neural Networks",
    author = "Dong, Li  and
      Wei, Furu  and
      Zhou, Ming  and
      Xu, Ke",
    booktitle = "Proceedings of the 53rd Annual Meeting of the Association for Computational Linguistics and the 7th International Joint Conference on Natural Language Processing (Volume 1: Long Papers)",
    month = jul,
    year = "2015",
    address = "Beijing, China",
    publisher = "Association for Computational Linguistics",
    url = "https://www.aclweb.org/anthology/P15-1026",
    doi = "10.3115/v1/P15-1026",
    pages = "260--269",
}

@inproceedings{fader-etal-2011-identifying,
    title = "Identifying Relations for Open Information Extraction",
    author = "Fader, Anthony  and
      Soderland, Stephen  and
      Etzioni, Oren",
    booktitle = "Proceedings of the 2011 Conference on Empirical Methods in Natural Language Processing",
    month = jul,
    year = "2011",
    address = "Edinburgh, Scotland, UK.",
    publisher = "Association for Computational Linguistics",
    url = "https://www.aclweb.org/anthology/D11-1142",
    pages = "1535--1545",
}

@inproceedings{sukhbaatar2015end,
  title={End-to-end memory networks},
  author={Sukhbaatar, Sainbayar and Weston, Jason and Fergus, Rob and others},
  booktitle={Advances in neural information processing systems},
  pages={2440--2448},
  year={2015}
}

@inproceedings{yang-etal-2014-joint,
    title = "Joint Relational Embeddings for Knowledge-based Question Answering",
    author = "Yang, Min-Chul  and
      Duan, Nan  and
      Zhou, Ming  and
      Rim, Hae-Chang",
    booktitle = "Proceedings of the 2014 Conference on Empirical Methods in Natural Language Processing ({EMNLP})",
    month = oct,
    year = "2014",
    address = "Doha, Qatar",
    publisher = "Association for Computational Linguistics",
    url = "https://www.aclweb.org/anthology/D14-1071",
    doi = "10.3115/v1/D14-1071",
    pages = "645--650",
}

@inproceedings{xu-etal-2016-question,
    title = "Question Answering on {F}reebase via Relation Extraction and Textual Evidence",
    author = "Xu, Kun  and
      Reddy, Siva  and
      Feng, Yansong  and
      Huang, Songfang  and
      Zhao, Dongyan",
    booktitle = "Proceedings of the 54th Annual Meeting of the Association for Computational Linguistics (Volume 1: Long Papers)",
    month = aug,
    year = "2016",
    address = "Berlin, Germany",
    publisher = "Association for Computational Linguistics",
    url = "https://www.aclweb.org/anthology/P16-1220",
    doi = "10.18653/v1/P16-1220",
    pages = "2326--2336",
}

@article{lehmann2015dbpedia,
  title={DBpedia--a large-scale, multilingual knowledge base extracted from Wikipedia},
  author={Lehmann, Jens and Isele, Robert and Jakob, Max and Jentzsch, Anja and Kontokostas, Dimitris and Mendes, Pablo N and Hellmann, Sebastian and Morsey, Mohamed and Van Kleef, Patrick and Auer, S{\"o}ren and others},
  journal={Semantic Web},
  volume={6},
  number={2},
  pages={167--195},
  year={2015},
  publisher={IOS Press}
}

@article{seaborne2008sparql,
  title={SPARQL/Update: A language for updating RDF graphs},
  author={Seaborne, Andy and Manjunath, Geetha and Bizer, Chris and Breslin, John and Das, Souripriya and Davis, Ian and Harris, Steve and Idehen, Kingsley and Corby, Olivier and Kjernsmo, Kjetil and others},
  journal={W3c member submission},
  volume={15},
  year={2008}
}

@article{dai2019transformer,
  title={Transformer-xl: Attentive language models beyond a fixed-length context},
  author={Dai, Zihang and Yang, Zhilin and Yang, Yiming and Cohen, William W and Carbonell, Jaime and Le, Quoc V and Salakhutdinov, Ruslan},
  journal={arXiv preprint arXiv:1901.02860},
  year={2019}
}

@inproceedings{yih-etal-2014-semantic,
    title = "Semantic Parsing for Single-Relation Question Answering",
    author = "Yih, Wen-tau  and
      He, Xiaodong  and
      Meek, Christopher",
    booktitle = "Proceedings of the 52nd Annual Meeting of the Association for Computational Linguistics (Volume 2: Short Papers)",
    month = jun,
    year = "2014",
    address = "Baltimore, Maryland",
    publisher = "Association for Computational Linguistics",
    url = "https://www.aclweb.org/anthology/P14-2105",
    doi = "10.3115/v1/P14-2105",
    pages = "643--648",
}

@inproceedings{yih-etal-2015-semantic,
    title = "Semantic Parsing via Staged Query Graph Generation: Question Answering with Knowledge Base",
    author = "Yih, Wen-tau  and
      Chang, Ming-Wei  and
      He, Xiaodong  and
      Gao, Jianfeng",
    booktitle = "Proceedings of the 53rd Annual Meeting of the Association for Computational Linguistics and the 7th International Joint Conference on Natural Language Processing (Volume 1: Long Papers)",
    month = jul,
    year = "2015",
    address = "Beijing, China",
    publisher = "Association for Computational Linguistics",
    url = "https://www.aclweb.org/anthology/P15-1128",
    doi = "10.3115/v1/P15-1128",
    pages = "1321--1331",
}

@inproceedings{yih-etal-2016-value,
    title = "The Value of Semantic Parse Labeling for Knowledge Base Question Answering",
    author = "Yih, Wen-tau  and
      Richardson, Matthew  and
      Meek, Chris  and
      Chang, Ming-Wei  and
      Suh, Jina",
    booktitle = "Proceedings of the 54th Annual Meeting of the Association for Computational Linguistics (Volume 2: Short Papers)",
    month = aug,
    year = "2016",
    address = "Berlin, Germany",
    publisher = "Association for Computational Linguistics",
    url = "https://www.aclweb.org/anthology/P16-2033",
    doi = "10.18653/v1/P16-2033",
    pages = "201--206",
}

@article{radford2018improving,
  title={Improving language understanding by generative pre-training},
  author={Radford, Alec and Narasimhan, Karthik and Salimans, Tim and Sutskever, Ilya},
  journal={URL https://s3-us-west-2. amazonaws. com/openai-assets/researchcovers/languageunsupervised/language understanding paper. pdf},
  year={2018}
}
@article{liu2019roberta,
  title={Roberta: A robustly optimized BERT pretraining approach},
  author={Liu, Yinhan and Ott, Myle and Goyal, Naman and Du, Jingfei and Joshi, Mandar and Chen, Danqi and Levy, Omer and Lewis, Mike and Zettlemoyer, Luke and Stoyanov, Veselin},
  journal={arXiv preprint arXiv:1907.11692},
  year={2019}
}

